Optimal Policy Synthesis from A Sequence of Goal Sets with An Application to Electric Distribution System Restoration

Motivated by the post-disaster distribution system restoration problem, in this paper, we study the problem of synthesizing the optimal policy for a Markov Decision Process (MDP) from a sequence of goal sets. For each goal set, our aim is to both maximize the probability to reach and minimize the expected time to reach the goal set. The order of the goal sets represents their priority. In particular, our aim is to generate a policy that is optimal with respect to the first goal set, and it is optimal with respect to the second goal set among the policies that are optimal with respect to the first goal set and so on. To synthesize such a policy, we iteratively filter the applicable actions according to the goal sets. We illustrate the developed method over sample distribution systems and disaster scenarios.

==> Sections/example/e1.tex <==



\begin{table}[ht]
  \begin{minipage}[b]{0.65\linewidth}
    \centering



\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-0.8,xscale=0.8]
%uncomment if require: \path (0,485); %set diagram left start at 0, and has height of 485

%Straight Lines [id:da8618963250953409] 
\draw    (390.23,70.24) -- (390.07,119.64) ;
%Rounded Rect [id:dp6213010722349394] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ][line width=0.75]  (304.41,68.69) .. controls (304.41,68.12) and (304.87,67.66) .. (305.44,67.66) -- (475.01,67.66) .. controls (475.58,67.66) and (476.04,68.12) .. (476.04,68.69) -- (476.04,71.78) .. controls (476.04,72.35) and (475.58,72.82) .. (475.01,72.82) -- (305.44,72.82) .. controls (304.87,72.82) and (304.41,72.35) .. (304.41,71.78) -- cycle ;
%Shape: Square [id:dp5863785149490699] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (386.29,77.05) -- (393.95,77.05) -- (393.95,84.71) -- (386.29,84.71) -- cycle ;
%Shape: Square [id:dp045091070594560634] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (386.38,106.29) -- (394.05,106.29) -- (394.05,113.95) -- (386.38,113.95) -- cycle ;
%Rounded Rect [id:dp615002391369306] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (360.89,118.22) .. controls (360.89,117.7) and (361.31,117.28) .. (361.83,117.28) -- (418.3,117.28) .. controls (418.82,117.28) and (419.24,117.7) .. (419.24,118.22) -- (419.24,121.05) .. controls (419.24,121.57) and (418.82,121.99) .. (418.3,121.99) -- (361.83,121.99) .. controls (361.31,121.99) and (360.89,121.57) .. (360.89,121.05) -- cycle ;
%Straight Lines [id:da9291343838891761] 
\draw    (390.18,54.6) -- (390.23,70.24) ;
%Straight Lines [id:da08932567037190531] 
\draw    (309.23,71.24) -- (309.07,120.64) ;
%Shape: Square [id:dp22421329565504866] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (305.29,78.05) -- (312.95,78.05) -- (312.95,85.71) -- (305.29,85.71) -- cycle ;
%Shape: Square [id:dp5448433291740307] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (305.38,107.29) -- (313.05,107.29) -- (313.05,114.95) -- (305.38,114.95) -- cycle ;
%Rounded Rect [id:dp8096604447519524] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (279.89,119.22) .. controls (279.89,118.7) and (280.31,118.28) .. (280.83,118.28) -- (337.3,118.28) .. controls (337.82,118.28) and (338.24,118.7) .. (338.24,119.22) -- (338.24,122.05) .. controls (338.24,122.57) and (337.82,122.99) .. (337.3,122.99) -- (280.83,122.99) .. controls (280.31,122.99) and (279.89,122.57) .. (279.89,122.05) -- cycle ;
%Straight Lines [id:da8539599913306865] 
\draw    (472.23,70.24) -- (472.07,119.64) ;
%Shape: Square [id:dp8588725074642922] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (468.29,77.05) -- (475.95,77.05) -- (475.95,84.71) -- (468.29,84.71) -- cycle ;
%Shape: Square [id:dp6397950747974741] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (468.38,106.29) -- (476.05,106.29) -- (476.05,113.95) -- (468.38,113.95) -- cycle ;
%Rounded Rect [id:dp2420267575739321] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (442.89,118.22) .. controls (442.89,117.7) and (443.31,117.28) .. (443.83,117.28) -- (500.3,117.28) .. controls (500.82,117.28) and (501.24,117.7) .. (501.24,118.22) -- (501.24,121.05) .. controls (501.24,121.57) and (500.82,121.99) .. (500.3,121.99) -- (443.83,121.99) .. controls (443.31,121.99) and (442.89,121.57) .. (442.89,121.05) -- cycle ;
%Straight Lines [id:da25945457888561585] 
\draw    (390.23,118.24) -- (390.07,167.64) ;
%Shape: Square [id:dp5460146293280694] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (386.29,125.05) -- (393.95,125.05) -- (393.95,132.71) -- (386.29,132.71) -- cycle ;
%Shape: Square [id:dp5495758836375766] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (386.38,154.29) -- (394.05,154.29) -- (394.05,161.95) -- (386.38,161.95) -- cycle ;
%Rounded Rect [id:dp44014233113618606] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (360.89,166.22) .. controls (360.89,165.7) and (361.31,165.28) .. (361.83,165.28) -- (418.3,165.28) .. controls (418.82,165.28) and (419.24,165.7) .. (419.24,166.22) -- (419.24,169.05) .. controls (419.24,169.57) and (418.82,169.99) .. (418.3,169.99) -- (361.83,169.99) .. controls (361.31,169.99) and (360.89,169.57) .. (360.89,169.05) -- cycle ;
%Straight Lines [id:da6129481665808583] 
\draw    (309.23,119.24) -- (309.07,168.64) ;
%Shape: Square [id:dp6554892952119263] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (305.29,126.05) -- (312.95,126.05) -- (312.95,133.71) -- (305.29,133.71) -- cycle ;
%Shape: Square [id:dp9314669483740932] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (305.38,155.29) -- (313.05,155.29) -- (313.05,162.95) -- (305.38,162.95) -- cycle ;
%Rounded Rect [id:dp5377463262969964] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (279.89,167.22) .. controls (279.89,166.7) and (280.31,166.28) .. (280.83,166.28) -- (337.3,166.28) .. controls (337.82,166.28) and (338.24,166.7) .. (338.24,167.22) -- (338.24,170.05) .. controls (338.24,170.57) and (337.82,170.99) .. (337.3,170.99) -- (280.83,170.99) .. controls (280.31,170.99) and (279.89,170.57) .. (279.89,170.05) -- cycle ;
%Straight Lines [id:da7009542593382363] 
\draw    (472.23,118.24) -- (472.07,167.64) ;
%Shape: Square [id:dp05659107128897278] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (468.29,125.05) -- (475.95,125.05) -- (475.95,132.71) -- (468.29,132.71) -- cycle ;
%Shape: Square [id:dp8468473835881949] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (468.38,154.29) -- (476.05,154.29) -- (476.05,161.95) -- (468.38,161.95) -- cycle ;
%Rounded Rect [id:dp0974615153155628] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (442.89,166.22) .. controls (442.89,165.7) and (443.31,165.28) .. (443.83,165.28) -- (500.3,165.28) .. controls (500.82,165.28) and (501.24,165.7) .. (501.24,166.22) -- (501.24,169.05) .. controls (501.24,169.57) and (500.82,169.99) .. (500.3,169.99) -- (443.83,169.99) .. controls (443.31,169.99) and (442.89,169.57) .. (442.89,169.05) -- cycle ;
%Straight Lines [id:da2990101079868619] 
\draw    (390.23,167.24) -- (390.07,216.64) ;
%Shape: Square [id:dp9867162775581106] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (386.29,174.05) -- (393.95,174.05) -- (393.95,181.71) -- (386.29,181.71) -- cycle ;
%Shape: Square [id:dp13637410880340284] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (386.38,203.29) -- (394.05,203.29) -- (394.05,210.95) -- (386.38,210.95) -- cycle ;
%Shape: Rectangle [id:dp5895447842365609] 
\draw   (372,32.67) -- (409.33,32.67) -- (409.33,54) -- (372,54) -- cycle ;
%Flowchart: Decision [id:dp895726539320798] 
\draw   (390.67,32.67) -- (409.33,43.33) -- (390.67,54) -- (372,43.33) -- cycle ;
%Straight Lines [id:da3515276970872637] 
\draw    (372,32.67) -- (409.33,54) ;
%Straight Lines [id:da12342902044929394] 
\draw    (409.33,32.67) -- (372,54) ;
%Rounded Rect [id:dp781088637082793] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ][line width=0.75]  (304.25,215.09) .. controls (304.25,214.52) and (304.71,214.06) .. (305.28,214.06) -- (474.85,214.06) .. controls (475.42,214.06) and (475.88,214.52) .. (475.88,215.09) -- (475.88,218.18) .. controls (475.88,218.75) and (475.42,219.21) .. (474.85,219.21) -- (305.28,219.21) .. controls (304.71,219.21) and (304.25,218.75) .. (304.25,218.18) -- cycle ;
%Straight Lines [id:da7023600461431544] 
\draw    (309.23,167.24) -- (309.07,216.64) ;
%Shape: Square [id:dp2635398486186704] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (305.29,174.05) -- (312.95,174.05) -- (312.95,181.71) -- (305.29,181.71) -- cycle ;
%Shape: Square [id:dp4535656826715865] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (305.38,203.29) -- (313.05,203.29) -- (313.05,210.95) -- (305.38,210.95) -- cycle ;
%Straight Lines [id:da009775871290058302] 
\draw    (472.23,167.24) -- (472.07,216.64) ;
%Shape: Square [id:dp6328471478419087] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (468.29,174.05) -- (475.95,174.05) -- (475.95,181.71) -- (468.29,181.71) -- cycle ;
%Shape: Square [id:dp6698899675404539] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (468.38,203.29) -- (476.05,203.29) -- (476.05,210.95) -- (468.38,210.95) -- cycle ;

% Text Node
\draw (345.13,59.09) node   [align=left] {1};
% Text Node
\draw (287.63,110.2) node   [align=left] {2};
% Text Node
\draw (367.67,109.67) node   [align=left] {4};
% Text Node
\draw (287,159.33) node   [align=left] {3};
% Text Node
\draw (449.67,158.67) node   [align=left] {8};
% Text Node
\draw (367.47,158.6) node   [align=left] {5};
% Text Node
\draw (347.8,206.93) node   [align=left] {6};
% Text Node
\draw (449.8,110.6) node   [align=left] {7};


\end{tikzpicture}

  \end{minipage}
  %\hfill
  \begin{varwidth}[b]{0.25\linewidth}
  {
      \renewcommand{\arraystretch}{1.2}
      \centering
      \begin{tabular}{c|c}
          Bus id & $P_f$ \\
          \hline
            1 & 0.125 \\
            2 & 0.500 \\ 
            3 & 0.250 \\ 
            4 & 0.500 \\ 
            5 & 0.500 \\ 
            6 & 0.500 \\ 
            7 & 0.125 \\ 
            8 & 0.125 \\ 
            \multicolumn{1}{c}{} \\
      \end{tabular}
    %\color{white}
    %\caption{
    %Probability of Failure
    %}
\hspace{0pt}
\vfill
  }
  \end{varwidth}%
  \vspace{8pt}
    \captionof{figure}{A distribution system and the probability of failure ($P_f$) values for each bus.}
    \label{fig:example_system1}
\end{table}

==> Sections/example/modified_example.tex <==
Consider the modified version of the system presented in figure \ref{fig:example_system}, where the bus 6 is connected to buses 3 and 8.
This system is depicted in figure \ref{fig:example_system1}, the remaining properties of the system ($P_f$ values and energy resources) are the same.
This modification increases the total state count from 126 to 196, 177 of which are terminal states.
The interesting consequence of this change is that there are multiple ways to reach a bus due to loops.

\input{Sections/example/e1}

Without changing $\textbf{B}$,
given that each energization attempt is successful, the optimal policy energizes the buses in this order: $\{1\}, \{7\}, \{2, 8\}, \{3, 4, 6\}, \{5\}$.
Instead of reaching bus 6 through 4 and 5, the optimal policy prefers the path through 7 and 8 since these buses have lower probability to fail.
$s_9 = {(E,U,U,U,U,U,D,U)}$ in this case (Tables \ref{transitions1:s9} and \ref{distances1:s9}) is analogous to $s_5$ in previous case (Tables \ref{transitions:s5} and \ref{distances:s5}); in both cases
the first energization attempt is successful and the second one is a failure.
Unlike before, the damaged component doesn't block the way thanks to loops, and there's still chance to energize both prioritized buses.


\begin{table}[H]
\centering
\caption{\\
Transitions from $s_{9} = {(E,U,U,U,U,U,D,U)}$
(System \ref{fig:example_system1})}
\begin{tabular} {c|c|c}
Action & Probability & Next State \\
\hline
\multirow{2}{*}{$\{4\}$} & 0.500 & $s_{41} = {(E,U,U,E,U,U,D,U)}$ \\
& 0.500 & $s_{21} = {(E,U,U,D,U,U,D,U)}$ \\
\hline
\multirow{2}{*}{$\{2\}$} & 0.500 & $s_{42} = {(E,E,U,U,U,U,D,U)}$ \\
& 0.500 & $s_{32} = {(E,D,U,U,U,U,D,U)}$ \\

\end{tabular}
\label{transitions1:s9}
\end{table}

\begin{table}[H]
\centering
\caption{Optimal values for $s_{9}$ (System \ref{fig:example_system1})}
\begin{tabular}{ l|l l l l }
Action & $P_{\infty, 1}^{\star}$ & $P_{\infty, 2}^{\star}$ & $C_{\infty, 1}^{\star}$ & $C_{\infty, 2}^{\star}$ \\
\hline
$\{4\}$ & $0.234375$ & -          & $3.800000$ & -          \\
$\{2\}$ & $0.234375$ & $0.453125$ & $3.400000$ & $2.344828$ 

\end{tabular}
\label{distances1:s9}
\end{table}

==> Sections/example/not_used_17.tex <==
\begin{table}[H]
\centering
\caption{Comparison of Algorithms for the System in Figure \ref{fig:mid_size}, for all priority sets $\{ i, j \}, i \neq j$ min-max}
\begin{tabular}{l l|p{0.2\linewidth} p{0.2\linewidth} p{0.2\linewidth}}
    & & Our Method & \cite{Arpali2019} & \cite{Gol2019} \\
                              \hline
    \multirow{4}{*}{$C_\infty^{G_1, \pi}$} 
    & mean & 5.2122 & 5.9602 & 5.9473 \\
    & std  & 1.2331 & 1.5404 & 1.5519 \\
    & min  & 1.0      & 1.0      & 1.0      \\
    & max  & 7.4060 & 8.3069 & 8.2541 \\
                              \hline
    \multirow{4}{*}{$C_\infty^{G_2, \pi}$} 
    & mean & 3.3624 & 3.4914 & 3.5041 \\
    & std  & 1.7393 & 1.8670 & 1.8928 \\
    & min  & 1.0      & 1.0      & 1.0      \\
    & max  & 6.7313 & 7.6108 & 7.6040 \\
                              \hline
    \multirow{4}{*}{$V_{17}^{\pi}$} 
    & mean & 209.0296 & 208.4996 & 208.6797 \\
    & std  &   0.354451 & 0.0        & 0.0         \\
    & min  & 208.6203 & 208.4996 & 208.6797 \\
    & max  & 210.3097 & 208.4996 & 208.6797 \\
\end{tabular}
\label{compare:mid_size1}
\end{table}



%%%%%%%%%%%



\begin{table}[H]
\centering
\caption{Comparison of Algorithms for the System in Figure \ref{fig:mid_size}, $B = [6, 12]$ min-max}
\begin{tabular}{l|p{0.2\linewidth} p{0.2\linewidth} p{0.2\linewidth}}
    \multirow{2}{*}{Goal Set} & \multicolumn{3}{c}{$C_\infty^{G_i, \pi}$ induced by $c_i$} \\
                              & Our Method & \cite{Arpali2019} & \cite{Gol2019} \\
                              \hline
    $G_1$                     &    6.394984 &       7.802508         &      8.846395\\
    $G_2$                     &    6.600886 &       7.544508         &      8.184208\\
\end{tabular}
\label{compare:mid_size1}
\end{table}

Next, in Table \ref{compare:mid_size2}, we demonstrate the case $\textbf{B} =[ \{3\}, \{6, 12\}]$, where $B_1 = \{3\}$ is in min-min, and $B_2 = \{6, 12\}$ is in min-max setting.
The goal sequence has 3 goal sets. The first one $G_1$ is the set of states which have bus 3 energized. Observe that there would be no difference in the goal sets or the goal sequence if it were min-max.
The remaining two goal sets are the same as the previous case, in the same order.
Note that the addition of another prioritization set ($\{ 3 \}$) negatively affected the expected times to reach other goal sets.

\begin{table}[H]
\centering
\caption{Comparison of Algorithms for the System in Figure \ref{fig:mid_size}, $\textbf{B} =[ \{3\}, \{6, 12\}]$, $B_1$ min-max, $B_2$ max-min}
\begin{tabular}{l|p{0.2\linewidth} p{0.2\linewidth} p{0.2\linewidth}}
    \multirow{2}{*}{Goal Set} & \multicolumn{3}{c}{$C_\infty^{G_i, \pi}$ induced by $c_i$} \\
                              & Our Method & \cite{Arpali2019} & \cite{Gol2019} \\
                              \hline
    $G_1$                     &    3.059107 &       4.059107         &      3.059107\\
    $G_2$                     &    7.241379 &       7.802508         &      8.846395\\
    $G_3$                     &    7.205253 &       7.544508         &      8.184208\\
\end{tabular}
\label{compare:mid_size2}
\end{table}

In the next case \ref{compare:mid_size3}, we extend the previous $B_1$ with bus 10.
$G_1$ becomes the set of states in which any of bus 3 or 10 is energized.
With this modification, it is still possible to reach $G_1$ if one of them becomes unreachable.
Due to this fact, the expected time to reach $G_1$ with our method is larger compared to previous case, since $C_\infty^{G_1, \pi}$ only considers the paths that reach the goal.
Besides, this change also increased the expected time to reach $G_2$ and $G_3$.
Because the policy tries to reach to bus 10 first if bus 3 turns out to be damaged/unreachable.
In the previous case, it would give up on $G_1$ if bus 3 is unreachable, and work towards $G_2$ and $G_3$.


\begin{table}[H]
\centering
\caption{Comparison of Algorithms for the System in Figure \ref{fig:mid_size}, $\textbf{B} =[ \{3, 10\}, \{6, 12\}]$, $B_1$ min-max, $B_2$ max-min}
\begin{tabular}{l|p{0.2\linewidth} p{0.2\linewidth} p{0.2\linewidth}}
    \multirow{2}{*}{Goal Set} & \multicolumn{3}{c}{$C_\infty^{G_i, \pi}$ induced by $c_i$} \\
                              & Our Method & \cite{Arpali2019} & \cite{Gol2019} \\
                              \hline
    $G_1$                     &    3.700849 &       4.498720         &    3.841926 \\
    $G_2$                     &    7.620298 &       7.802508         &    8.846395 \\
    $G_3$                     &    7.562127 &       7.544509         &    8.184208 \\
\end{tabular}
\label{compare:mid_size3}
\end{table}



==> Sections/example/old_e0.tex <==

% \begin{figure}[h]
% \begin{tikzpicture}[auto,node distance=8mm,>=latex,font=\small]
% \tikzstyle{round}=[thick,draw=black,circle]
% \begin{scope}[local bounding box=graph]
% \node[round, label=south:$0.125$, label=0:{Connected to $E_{0}$}] (0) at (0,0) {1};
% \node[round, label=south:$0.500$] (1) at (-1.4743094474174336,1.342529328579414) {2};
% \node[round, label=south:$0.250$] (2) at (-3.355324949294849,1.3808858626923248) {3};
% \node[round, label=south:$0.500$] (3) at (-2.2368832995309513,-0.20138378215128233) {4};
% \node[round, label=south:$0.500$] (4) at (-4.359380521242929,-0.5754042953834736) {5};
% \node[round, label=south:$0.500$] (5) at (-6.0497525600922275,-0.901459180366965) {6};
% \node[round, label=south:$0.125$] (6) at (-1.0803129571593264,-1.5729325336308235) {7};
% \node[round, label=south:$0.125$] (7) at (-3.113843229460287,-2.0715042723501598) {8};
% \draw[-] (0) -- (3);
% \draw[-] (3) -- (4);
% \draw[-] (4) -- (5);
% \draw[-] (0) -- (1);
% \draw[-] (1) -- (2);
% \draw[-] (0) -- (6);
% \draw[-] (6) -- (7);
% \end{scope}
% \end{tikzpicture}
% \caption{Example Distribution System}
% \label{exampledist}
% \end{figure}




\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,394); %set diagram left start at 0, and has height of 394

%Rounded Rect [id:dp2426241565626941] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ][line width=0.75]  (282.83,120.59) .. controls (282.83,119.98) and (283.32,119.49) .. (283.93,119.49) -- (340.53,119.49) .. controls (341.13,119.49) and (341.63,119.98) .. (341.63,120.59) -- (341.63,123.89) .. controls (341.63,124.5) and (341.13,124.99) .. (340.53,124.99) -- (283.93,124.99) .. controls (283.32,124.99) and (282.83,124.5) .. (282.83,123.89) -- cycle ;
%Straight Lines [id:da5993624015309964] 
\draw    (312.23,122.24) -- (312.07,171.64) ;
%Rounded Rect [id:dp293025361022629] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ][line width=0.75]  (253.04,170.16) .. controls (253.04,169.62) and (253.48,169.18) .. (254.02,169.18) -- (370.11,169.18) .. controls (370.65,169.18) and (371.1,169.62) .. (371.1,170.16) -- (371.1,173.11) .. controls (371.1,173.65) and (370.65,174.1) .. (370.11,174.1) -- (254.02,174.1) .. controls (253.48,174.1) and (253.04,173.65) .. (253.04,173.11) -- cycle ;
%Shape: Square [id:dp7246313378653004] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (308.29,129.05) -- (315.95,129.05) -- (315.95,136.71) -- (308.29,136.71) -- cycle ;
%Shape: Square [id:dp6296074484082603] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (308.38,158.29) -- (316.05,158.29) -- (316.05,165.95) -- (308.38,165.95) -- cycle ;
%Rounded Rect [id:dp8860324618586426] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (242.22,222.28) .. controls (242.22,221.77) and (242.63,221.35) .. (243.15,221.35) -- (320.74,221.35) .. controls (321.25,221.35) and (321.67,221.77) .. (321.67,222.28) -- (321.67,225.07) .. controls (321.67,225.58) and (321.25,226) .. (320.74,226) -- (243.15,226) .. controls (242.63,226) and (242.22,225.58) .. (242.22,225.07) -- cycle ;
%Rounded Rect [id:dp27051227409909706] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (341.36,221.8) .. controls (341.36,221.28) and (341.78,220.86) .. (342.3,220.86) -- (398.77,220.86) .. controls (399.29,220.86) and (399.71,221.28) .. (399.71,221.8) -- (399.71,224.63) .. controls (399.71,225.15) and (399.29,225.57) .. (398.77,225.57) -- (342.3,225.57) .. controls (341.78,225.57) and (341.36,225.15) .. (341.36,224.63) -- cycle ;
%Straight Lines [id:da5721527896412115] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ]   (271.5,172.8) -- (271.12,222.1) ;
%Straight Lines [id:da7123453435287654] 
\draw    (370.11,174.1) -- (370.28,223.1) ;
%Rounded Rect [id:dp5994951863758078] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (214.68,272.88) .. controls (214.68,272.35) and (215.11,271.92) .. (215.64,271.92) -- (272.47,271.92) .. controls (273,271.92) and (273.43,272.35) .. (273.43,272.88) -- (273.43,275.75) .. controls (273.43,276.28) and (273,276.71) .. (272.47,276.71) -- (215.64,276.71) .. controls (215.11,276.71) and (214.68,276.28) .. (214.68,275.75) -- cycle ;
%Straight Lines [id:da5558077055825197] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ]   (320.74,226) -- (320.9,275) ;
%Rounded Rect [id:dp3670915876024279] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (303.22,272.71) .. controls (303.22,272.19) and (303.63,271.78) .. (304.15,271.78) -- (381.74,271.78) .. controls (382.25,271.78) and (382.67,272.19) .. (382.67,272.71) -- (382.67,275.5) .. controls (382.67,276.01) and (382.25,276.43) .. (381.74,276.43) -- (304.15,276.43) .. controls (303.63,276.43) and (303.22,276.01) .. (303.22,275.5) -- cycle ;
%Straight Lines [id:da2303319039484244] 
\draw    (381.57,222.78) -- (381.74,271.78) ;
%Straight Lines [id:da26707234511587763] 
\draw    (243.92,225.67) -- (244.08,274.67) ;
%Shape: Square [id:dp557282175930544] 
\draw  [fill={rgb, 255:red, 65; green, 117; blue, 5 }  ,fill opacity=1 ] (267.81,178.29) -- (275.48,178.29) -- (275.48,185.95) -- (267.81,185.95) -- cycle ;
%Shape: Square [id:dp8218113681467967] 
\draw  [fill={rgb, 255:red, 65; green, 117; blue, 5 }  ,fill opacity=1 ] (267.52,210) -- (275.19,210) -- (275.19,217.67) -- (267.52,217.67) -- cycle ;
%Shape: Square [id:dp015476401883822266] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (366.38,179.43) -- (374.05,179.43) -- (374.05,187.1) -- (366.38,187.1) -- cycle ;
%Shape: Square [id:dp3323975538336237] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (366.38,209.71) -- (374.05,209.71) -- (374.05,217.38) -- (366.38,217.38) -- cycle ;
%Shape: Square [id:dp4741904377669688] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (240.38,230.29) -- (248.05,230.29) -- (248.05,237.95) -- (240.38,237.95) -- cycle ;
%Shape: Square [id:dp35450514122487653] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (240.38,260.86) -- (248.05,260.86) -- (248.05,268.52) -- (240.38,268.52) -- cycle ;
%Shape: Square [id:dp7903714392899321] 
\draw  [fill={rgb, 255:red, 65; green, 117; blue, 5 }  ,fill opacity=1 ] (316.95,230.86) -- (324.62,230.86) -- (324.62,238.52) -- (316.95,238.52) -- cycle ;
%Shape: Square [id:dp7310091053085304] 
\draw  [fill={rgb, 255:red, 65; green, 117; blue, 5 }  ,fill opacity=1 ] (316.95,261.14) -- (324.62,261.14) -- (324.62,268.81) -- (316.95,268.81) -- cycle ;
%Shape: Square [id:dp6969020758554965] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (377.81,229.71) -- (385.48,229.71) -- (385.48,237.38) -- (377.81,237.38) -- cycle ;
%Shape: Square [id:dp5626005948937072] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (378.1,261.57) -- (385.76,261.57) -- (385.76,269.24) -- (378.1,269.24) -- cycle ;
%Straight Lines [id:da9815681847678597] 
\draw    (170,149.4) -- (170.2,271.4) ;
%Straight Lines [id:da039234422489200727] 
\draw    (140.7,170.6) -- (189.4,170.2) ;

% Text Node
\draw (289.13,113.09) node   [align=left] {1};
% Text Node
\draw (263.63,161.2) node   [align=left] {2};
% Text Node
\draw (250.67,211.67) node   [align=left] {3};
% Text Node
\draw (349,213.33) node   [align=left] {5};
% Text Node
\draw (311.67,265.67) node   [align=left] {4};
% Text Node
\draw (223.47,263.6) node   [align=left] {6};
% Text Node
\draw (334.5,145.5) node   [align=left] {{\scriptsize Branch-0}};
% Text Node
\draw (392.5,197.5) node  [font=\scriptsize] [align=left] {Branch-1};
% Text Node
\draw (293,196.5) node  [font=\scriptsize] [align=left] {Branch-2};
% Text Node
\draw (342.5,249.5) node  [font=\scriptsize] [align=left] {Branch-3};
% Text Node
\draw (403.5,251) node  [font=\scriptsize] [align=left] {ranch-4};
% Text Node
\draw (266,249) node  [font=\scriptsize] [align=left] {Branch-5};
% Text Node
\draw (157,154.7) node   [align=left] {\begin{minipage}[lt]{19.040000000000003pt}\setlength\topsep{0pt}
{\scriptsize node}
\end{minipage}};
% Text Node
\draw (181,155) node   [align=left] {\begin{minipage}[lt]{17.68000000000001pt}\setlength\topsep{0pt}
{\scriptsize P\_f}
\end{minipage}};
% Text Node
\draw (180,220.6) node   [align=left] {\begin{minipage}[lt]{10.608000000000017pt}\setlength\topsep{0pt}
{\scriptsize 0.1}\\{\scriptsize 0.2}\\{\scriptsize 0.3}\\{\scriptsize 0.4}\\{\scriptsize 0.5}
\end{minipage}};
% Text Node
\draw (155.8,220.2) node   [align=left] {\begin{minipage}[lt]{8.67pt}\setlength\topsep{0pt}
{\scriptsize 1}\\{\scriptsize 2}\\{\scriptsize 3}\\{\scriptsize 4}\\{\scriptsize 5}
\end{minipage}};


\end{tikzpicture}


==> Sections/example/s1.tex <==


\begin{table}[h]
\centering
\caption{Transitions from $s_{1} = {(U,U,U,U,U,U,U,U)}$}
\begin{tabular} {c|c|c}
Action & Probability & Next State \\
\hline
\multirow{2}{*}{$\{1\}$} & 0.875 & $s_{2} = {(E_0,U,U,U,U,U,U,U)}$ \\
& 0.125 & $s_{3} = {(D,U,U,U,U,U,U,U)}$ \\

\end{tabular}
\label{transitions:s1}
\end{table}

\begin{table}[h]
\centering
\caption{Optimal values for $s_{1}$}
\begin{tabular}{ l|l l l l l }
Action & $P_{\infty, 1,2}^{\star}$ & $P_{\infty, 1,1}^{\star}$ & $C_{\infty, 1,2}^{\star}$ & $C_{\infty, 1,1}^{\star}$ & $V$ \\
\hline
$\{1\}$ & $0.202728$ & $0.415070$ & $4.681770$ & $4.138960$ & $39.990520$ \\

\end{tabular}
\label{distances:s1}
\end{table}




\begin{table}[h]
\centering
\caption{Transitions from $s_{2} = {(E_0,U,U,U,U,U,U,U)}$}
\begin{tabular} {c|c|c}
Action & Probability & Next State \\
\hline
\multirow{2}{*}{$\{4\}$} & 0.500 & $s_{4} = {(E_0,U,U,E_0,U,U,U,U)}$ \\
& 0.500 & $s_{5} = {(E_0,U,U,D,U,U,U,U)}$ \\
\hline
\multirow{2}{*}{$\{2\}$} & 0.500 & $s_{6} = {(E_0,E_0,U,U,U,U,U,U)}$ \\
& 0.500 & $s_{7} = {(E_0,D,U,U,U,U,U,U)}$ \\
\hline
\multirow{2}{*}{$\{7\}$} & 0.875 & $s_{8} = {(E_0,U,U,U,U,U,E_0,U)}$ \\
& 0.125 & $s_{9} = {(E_0,U,U,U,U,U,D,U)}$ \\

\end{tabular}
\label{transitions:s2}
\end{table}

\begin{table}[h]
\centering
\caption{Optimal values for $s_{2}$}
\begin{tabular}{ l|l l l l l }
Action & $P_{\infty, 1,2}^{\star}$ & $P_{\infty, 1,1}^{\star}$ & $C_{\infty, 1,2}^{\star}$ & $C_{\infty, 1,1}^{\star}$ & $V$ \\
\hline
$\{4\}$ & $0.231689$ & $0.570068$ & $3.968388$ & $3.822440$ & $33.733824$ \\
$\{2\}$ & $0.231689$ & $0.475342$ & $4.170706$ & $3.622748$ & $33.496411$ \\
$\{7\}$ & $0.231689$ & $0.474365$ & $3.681770$ & $3.138960$ & $32.640696$ \\

\end{tabular}
\label{distances:s2}
\end{table}



\begin{table}[h]
\centering
\caption{Transitions from $s_{8} = {(E_0,U,U,U,U,U,E_0,U)}$}
\begin{tabular} {c|c|c}
Action & Probability & Next State \\
\hline
\multirow{4}{*}{$\{4, 8\}$} & 0.438 & $s_{33} = {(E_0,U,U,E_0,U,U,E_0,E_0)}$ \\
& 0.063 & $s_{34} = {(E_0,U,U,E_0,U,U,E_0,D)}$ \\
& 0.438 & $s_{35} = {(E_0,U,U,D,U,U,E_0,E_0)}$ \\
& 0.063 & $s_{36} = {(E_0,U,U,D,U,U,E_0,D)}$ \\
\hline
\multirow{4}{*}{$\{2, 8\}$} & 0.438 & $s_{37} = {(E_0,E_0,U,U,U,U,E_0,E_0)}$ \\
& 0.063 & $s_{38} = {(E_0,E_0,U,U,U,U,E_0,D)}$ \\
& 0.438 & $s_{39} = {(E_0,D,U,U,U,U,E_0,E_0)}$ \\
& 0.063 & $s_{40} = {(E_0,D,U,U,U,U,E_0,D)}$ \\

\end{tabular}
\label{transitions:s8}
\end{table}

\begin{table}[h]
\centering
\caption{Optimal values for $s_{8}$}
\begin{tabular}{ l|l l l l l }
Action & $P_{\infty, 1,2}^{\star}$ & $P_{\infty, 1,1}^{\star}$ & $C_{\infty, 1,2}^{\star}$ & $C_{\infty, 1,1}^{\star}$ & $V$ \\
\hline
$\{4, 8\}$ & $0.240234$ & $0.486328$ & $2.593496$ & $2.072289$ & $27.445261$ \\
$\{2, 8\}$ & $0.240234$ & $0.589844$ & $3.065041$ & $2.738956$ & $27.344324$ \\

\end{tabular}
\label{distances:s8}
\end{table}




\begin{table}[h]
\centering
\caption{Transitions from $s_{33} = {(E_0,U,U,E_0,U,U,E_0,E_0)}$}
\begin{tabular} {c|c|c}
Action & Probability & Next State \\
\hline
\multirow{8}{*}{$\{2, 5, 6\}$} & 0.125 & $s_{61} = {(E_0,E_0,U,E_0,E_0,E_0,E_0,E_0)}$ \\
& 0.125 & $s_{63} = {(E_0,E_0,U,E_0,E_0,D,E_0,E_0)}$ \\
& 0.125 & $s_{117} = {(E_0,E_0,U,E_0,D,E_0,E_0,E_0)}$ \\
& 0.125 & $s_{118} = {(E_0,E_0,U,E_0,D,D,E_0,E_0)}$ \\
& 0.125 & $s_{65} = {(E_0,D,U,E_0,E_0,E_0,E_0,E_0)}$ \\
& 0.125 & $s_{67} = {(E_0,D,U,E_0,E_0,D,E_0,E_0)}$ \\
& 0.125 & $s_{119} = {(E_0,D,U,E_0,D,E_0,E_0,E_0)}$ \\
& 0.125 & $s_{120} = {(E_0,D,U,E_0,D,D,E_0,E_0)}$ \\

\end{tabular}
\label{transitions:s33}
\end{table}

\begin{table}[h]
\centering
\caption{Optimal values for $s_{33}$}
\begin{tabular}{ l|l l l l l }
Action & $P_{\infty, 1,2}^{\star}$ & $P_{\infty, 1,1}^{\star}$ & $C_{\infty, 1,2}^{\star}$ & $C_{\infty, 1,1}^{\star}$ & $V$ \\
\hline
$\{2, 5, 6\}$ & $0.250000$ & $0.500000$ & $1.000000$ & $1.000000$ & $18.054669$ \\

\end{tabular}
\label{distances:s33}
\end{table}



\begin{table}[h]
\centering
\caption{Transitions from $s_{61} = {(E_0,E_0,U,E_0,E_0,E_0,E_0,E_0)}$}
\begin{tabular} {c|c|c}
Action & Probability & Next State \\
\hline
\multirow{2}{*}{$\{3\}$} & 0.750 & $s_{137} = {(E_0,E_0,E_0,E_0,E_0,E_0,E_0,E_0)}$ \\
& 0.250 & $s_{141} = {(E_0,E_0,D,E_0,E_0,E_0,E_0,E_0)}$ \\
\hline
\multirow{2}{*}{$\{3\}$} & 0.750 & $s_{137} = {(E_0,E_0,E_0,E_0,E_0,E_0,E_0,E_0)}$ \\
& 0.250 & $s_{141} = {(E_0,E_0,D,E_0,E_0,E_0,E_0,E_0)}$ \\

\end{tabular}
\label{transitions:s61}
\end{table}

\begin{table}[h]
\centering
\caption{Optimal values for $s_{61}$}
\begin{tabular}{ l|l }
Action & $V$ \\
\hline
$\{3\}$ & $2.749998$ \\
$\{3\}$ & $2.749998$ \\

\end{tabular}
\label{distances:s61}
\end{table}






==> Sections/problem_formulation.tex <==


\subsection{Problem Formulation}%
\label{sub:problem_formulation}

The optimal policy must satisfy the following:

\begin{equation} \label{eq:mingoal1}
    \pi^*(s) \in \argmin_{\pi \in A^S} D_\infty^{G_1, \pi}(s)
\end{equation}

Depending on the problem, there might be many policies that satisfy this condition.
In that case, the optimal policy must minimize the expected time steps to reach $G_2$ as well:

\begin{equation} \label{eq:mingoal2}
    \pi^*(s) \in
    \argmin_{\pi: \forall s' \in S, \pi(s') \in \argmin_{\pi \in A^S} D_\infty^{G_1, \pi}(s')}
    D_\infty^{G_2, \pi} (s)
\end{equation}

This will continue in a recursive fashion until all goal sets in the given sequence $G_s$ are exhausted.
Finally, the optimal policy will be the one that minimizes the value function among all policies that satisfy the previous conditions.

\begin{equation*}
    \Pi_0 = A^S
\end{equation*}
\begin{equation*}
    \Pi_i = \{ \pi \mid \forall s \in S, \argmin_{\pi \in \Pi_{i-1}} D_\infty^{G_i, \pi}(s) \}
\end{equation*}

\begin{equation*}
    \pi^* (s) \in\argmin_{\pi \in \Pi_{|G_s|}} D_\infty^{G_i, \pi}(s) 
\end{equation*}


